MolmoAct: Action Reasoning Models that can Reason in Space

Reasoning is central to purposeful action, yet most robotic foundation models map perception and instructions directly to control, which limits adaptability, generalization, and semantic grounding. We introduce Action Reasoning Models (ARMs), a class of robotic foundation models that integrate perception, planning, and control through a structured three-stage pipeline. Our model, MolmoAct, encodes observations and instructions into depth-aware perception tokens, generates mid-level spatial plans as editable trajectory traces, and predicts precise low-level actions, enabling explainable and steerable behavior. MolmoAct-7B-D achieves strong performance across simulation and real-world settings: 70.5% zero-shot accuracy on SimplerEnv Visual Matching tasks, surpassing closed-source Pi-0 and GR00T N1.5; 86.6% average success on LIBERO, including an additional 6.3% gain over ThinkAct on long-horizon tasks; and in real-world fine-tuning, an additional 10% (single-arm) and an additional 22.7% (bimanual) task progression over Pi-0-FAST. It also outperforms baselines by an additional 23.3% on out-of-distribution generalization and achieves top human-preference scores for open-ended instruction following and trajectory steering. Furthermore, we release, for the first time, the MolmoAct Dataset -- a mid-training robot dataset comprising over 10,000 high quality robot trajectories across diverse scenarios and tasks. Training with this dataset yields an average 5.5% improvement in general performance over the base model. We release all model weights, training code, our collected dataset, and our action reasoning dataset, establishing MolmoAct as both a state-of-the-art robotics foundation model and an open blueprint for building ARMs that transform perception into purposeful action through structured reasoning. Blogpost: https://allenai.org/blog/molmoact

==> ai2style/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> sections/old/1-introduction-v1.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]  % spans both columns
  \centering
  \includegraphics[width=\textwidth]{figures/MolmoAct_V7.pdf}
  \caption{\textbf{Overview}. \textsc{MolmoAct} is an open action reasoning model that, given a user’s language instruction, reasons in space and autoregressively predicts three structured reasoning chains: \textsc{Depth Perception Tokens} for sensing and reconstructing the 3D environment, \textsc{Visual Reasoning Trace Tokens} for representing its planned trajectory in the scene, and \textsc{Action Tokens} for generating the corresponding robot control commands. Each reasoning chain can be independently decoded—yielding a depth map of the scene, a 2D trajectory overlay on the image plane, and executed actions in the physical world—providing explicit, spatially grounded reasoning at every stage.}
  \label{fig:full_width_image}
\end{figure*}

\begin{quote}
  \textit{The mind is inherently embodied; thought is not merely a matter of logic or language—it is grounded in the body’s interactions with the world.}\\[2pt]
  --- George Lakoff \& Mark Johnson, \emph{Philosophy in the Flesh}
\end{quote}


Reasoning allows us to act with intention. Before reaching for a cup or moving through a room, we subconsciously weigh context, goals, and constraints—transforming perception into purpose. This deliberative process, grounded in our physical experience of the world, makes our actions coherent, adaptable, and interpretable. For robots to operate with the same fluency, they must do more than map images and instructions to control commands. They must learn to reason.

In contrast to the rapid generalization gains seen in large language and vision models, progress in robotics has lagged behind \citep{duan2022survey,xu2024survey,firoozi2025foundation}. Vision-Language-Action (VLA) models aim to bring similar capabilities to physical agents, but have yet to reach the same level of flexibility or robustness. Despite massive efforts in dataset collection and model scaling, today's VLAs remain brittle and opaque—struggling to transfer across tasks, scenes, or embodiments, and offering little insight into why a robot chose one action over another \citep{liu2025towards,pumacay2024colosseum}.



This gap stems not just from limited data, but from a lack of structure. While language and vision tasks benefit from abundant, loosely labeled web-scale data, robotics demands fine-grained, embodied interaction—data that is costly, ambiguous, and difficult to scale. Yet in parallel, language models have begun to shift away from brute-force scaling toward \textit{structured learning}: building intermediate representations that support reasoning, abstraction, and control \citep{wei2022chain,zelikman2022star,huang2022large}. We believe robotics can—and must—do the same.

We introduce \textsc{\textsc{MolmoAct}} (\textbf{M}ultimodal \textbf{O}pen \textbf{L}anguage \textbf{Mo}del for \textbf{Act}ion), a family of completely open \textbf{A}ction \textbf{R}easoning \textbf{M}odels (\textbf{ARM}) that integrate perception, planning, and control through a structured reasoning pipeline. \textsc{MolmoAct} learns to interpret language instructions, sense its environment, generate spatial plans, and execute them as smooth, goal-directed trajectories. The model first encodes observations and instructions into structured 2.5D representations via autoregressive prediction of depth-aware perception tokens. These tokens condition the generation of mid-level planning representations—visualized as trajectory lines in image space—which then guide the prediction of precise, low-level robot actions. This three-stage reasoning architecture enables \textsc{MolmoAct} to produce interpretable, spatially coherent behavior.

\textsc{MolmoAct}’s structured design delivers both strong performance and high transparency. On standard benchmarks such as LIBERO and SimPLER (Fractal), \textsc{MolmoAct} consistently outperforms competitive baselines including GROOT \citep{nvidia2025gr00tn1openfoundation}, Pi-0 \citep{black2410pi0}, RT-1 \citep{brohan2022rt}, and TraceVLA \citep{zheng2024tracevla}. In arena-style human evaluations for open-ended language instruction following, \textsc{MolmoAct} is preferred over baselines, achieving significantly higher Elo ratings. The model adapts to novel tasks more effectively through lightweight fine-tuning, surpassing other strong baselines in efficiency. Moreover, it generalizes well to diverse environments and task perturbations in both simulation and real-world settings. Its visual reasoning traces offer an interpretable view into the model’s decision-making, while also enabling direct action steering by editing trajectory lines—an approach we find more reliable than language commands, which can suffer from ambiguity.


\textsc{MolmoAct} is fully open in every aspect: we release the model weights, training code, and all components of our multimodal reasoning dataset. We aim for \textsc{MolmoAct} to be more than a high performing robotics foundation model that serves as a blueprint for building agents that reason, transforming perception into purposeful action through reasoning.





% \section{Introduction}
% \label{sec:intro}

% \begin{quote}
%   \textit{The mind is inherently embodied; thought is not merely a matter of logic or language—it is grounded in the body’s interactions with the world.}\\[2pt]
%   --- George Lakoff \& Mark Johnson, \emph{Philosophy in the Flesh}
% \end{quote}

% Reasoning stands as one of humanity's most profound endowments, conferred upon us throughout the intricate course of our developmental journey. It equips us with the cognitive faculties to deliberate, strategize, and articulate our thoughts coherently before engaging in action. Furthermore, reasoning engenders a unique openness whereby cognitive processes are systematically grounded, fostering clarity and coherence in our understanding of an agent’s internal deliberations and behaviors. This transparency mitigates uncertainty and fear, for apprehension arises predominantly from ignorance.

% With remarkable advancements in scaling data within the language and vision domains, the world has witnessed the rise of intelligent general-purpose foundation models. These foundation models, pre-trained to function as versatile agents, possess the remarkable capacity to swiftly adapt and specialize within targeted domains. Such paradigms of pre-training have catalyzed efforts aimed at replicating analogous successes within robotics, thus prompting the emergence of Vision-Language-Action models (VLAs). Regrettably, pre-training exclusively on robotic data has yet to yield a comparable degree of generalizability and interactive proficiency as exhibited by contemporary large language models (LLMs) or vision-language models (VLMs). Furthermore, extensive training on laboriously accumulated robotic datasets alone falls short of eliciting the emergent properties and transformative successes achieved by LLMs and VLMs. 

% In recent years, faced with the dwindling availability of new data for pre-training LLMs, researchers have increasingly focused on leveraging existing data through compositional and rationalized learning methods. Robotics faces a similar dilemma, albeit from a different perspective. Current VLA models predominantly adopt an end-to-end strategy, characterized by a straightforward approach of robot data input leading directly to actions. Given the substantial costs and intensive labor involved in collecting physical-world robot data, scaling robotics models often devolves into a resource-intensive exercise in data acquisition. Thus arises a critical inquiry: Can reasoning, when applied effectively to existing data, facilitate the pre-training of robotic models that exhibit enhanced generalizability, interactivity, and interpretability? Addressing this question entails grappling with a series of significant challenges inherent to the development of robust generalist robotic reasoning models. First, How can we efficiently train a robust, open‑world generalist robotics model that fully exploits large‑scale pre‑training? Second, What is the right way to perform reasoning on robotics data—fundamentally different from language data which is far less ambiguous? Third, How do we rigorously measure the advantages of action‑reasoning models in solving tasks, and what new capabilities and properties do they unlock?



% We present \textbf{\textsc{MolmoAct}} (\textbf{M}ultimodal \textbf{O}pen \textbf{L}anguage \textbf{Mo}del for \textbf{Act}ion), a fully open‑sourced family of action reasoning models. Alongside the model weights, we release the entire multimodal training corpus—including every stage of robot action‑reasoning data—and our proprietary \textsc{MolmoAct} dataset, which spans over 100 tasks collected in diverse real‑world scenes. \textsc{MolmoAct}’s success rests on a three‑tier curriculum: (i) meticulously filtered large‑scale pre‑training data from Open-X embodiment dataset, (ii) high‑quality post-training data, and (iii) a unified robot action reasoning data that grounds the model’s reasoning in physical interactions. \textbf{\textsc{MolmoAct}} is a fully open‑source action‑reasoning model that consistently surpasses leading VLA baselines—including Groot, Pi\_0, RT‑1, and TraceVLA—on major simulation benchmarks such as Libero, SimPLER (Fractal), and RoboEval. These results demonstrate \textsc{MolmoAct}’s strength as a general‑purpose robotics solution: it excels at multi‑task performance, remains robust to environmental perturbations, and adapts readily to diverse robot embodiments. Extensive real‑world tests on both single‑arm and bimanual Franka platforms confirm the same performance advantages. 

% Beyond being a robust and capable generalist robotics model, \textbf{\textsc{MolmoAct}} uniquely integrates spatial reasoning, enabling it to generate smooth and high-quality robot trajectories. When evaluated using RoboEval, \textbf{\textsc{MolmoAct}} significantly outperforms baseline methods. Additionally, our instruction-following human evaluations conducted through an arena-style simulation demonstrate that \textbf{\textsc{MolmoAct}} achieves notably higher Elo ratings, reflecting strong human preference for its ability to follow instructions accurately. The success of \textbf{\textsc{MolmoAct}}'s reasoning capability can be largely attributed to our curated robot reasoning dataset. This dataset grounds the reasoning process by first converting observations and language instructions into a structured 2.5D perception representation. Specifically, \textbf{\textsc{MolmoAct}} is autoregressively trained to predict perception tokens that encapsulate scene understanding. These perception tokens then condition the model to generate planning representations, visualized as trajectory lines on the image plane. This intermediate representation guides the final step of predicting precise robot actions.

% One of the significant drawbacks of existing general-purpose robotics models is their unpredictability, as humans interacting with these robots often cannot understand the model's intentions or anticipate its actions. \textbf{\textsc{MolmoAct}} addresses this issue uniquely by offering complete transparency—our code, weights, and datasets are openly available, and the model explicitly communicates its intended actions at each timestep through visualized trajectory lines. Furthermore, \textbf{\textsc{MolmoAct}} provides enhanced steerability, enabling users to interactively guide robot actions in real-time by drawing trajectory lines directly onto images. This visual steering method offers clear, grounded communication compared to language instructions, which can be ambiguous, thus ensuring that robot behavior aligns closely with user intentions.




==> tables/midtrain_mixes.tex <==
\newcommand{\MeBaseline}{{\sans{PT Mix}}\xspace}
\newcommand{\MeDclmSeven}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}$\xspace}
\newcommand{\MeFinewebThree}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{3}}}}$\xspace}
\newcommand{\MeFinewebTwo}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}$\xspace}
\newcommand{\MeFinewebTwoMath}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Math}\xspace}
\newcommand{\MeFinewebTwoIns}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Ins}\xspace}
\newcommand{\MeFinewebTwoMathIns}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Math + Ins}\xspace}


\begin{table}[ht]
\renewcommand{\arraystretch}{.9}
\setlength\tabcolsep{3pt}
\begin{center}
\begin{footnotesize}
\newcommand{\rot}[1]{\rotatebox{90}{#1}}
\begin{tabular}{c @{\hskip 6pt} l @{\hskip 6pt} l c c c c c c c}
\toprule
    & \multirow{2}{*}{\vspace{-1.5em}\textbf{\footnotesize{Source}}} 
    &
    & \multicolumn{7}{c}{\textbf{\footnotesize~Mix \%}} 
    \vspace{.5em}
    \\[-.3em]
    &
    &
    &
    \MeBaseline &
    \MeDclmSeven &
    \MeFinewebThree &
    \MeFinewebTwo &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Math}}
    } &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Ins}}
    } &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Math}}
        \\[-.2em]
        {\sans{+ Ins}}
    }
    \\
\midrule
    \rowcolor{ai2offwhite}
    &
    \sans{DCLM} & 
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    95.2 & 
    - & 
    - & 
    - & 
    - & 
    - & 
    - 
\\
    \rowcolor{ai2offwhite}
    & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}\\
    \end{tabular} & 
    - &
    57.1 &
    - &
    - &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}
    & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}
        \\[-.4em]
        {\scriptsize\color{darkergrey}$\text{FineWeb}\geqslant3$}
    \end{tabular} & 
    - &
    - &
    54.2 &
    - &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}
    \multirow{-4}{*}{\rot{\textbf{\hspace{2em}\scriptsize{WEB}}}} & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}
        \\[-.4em]
        {\scriptsize\color{darkergrey}$\text{FineWeb}\geqslant2$}
    \end{tabular} & 
    - &
    - &
    - &
    57.9 &
    61.8 &
    75.5 &
    57.5
\\
    &
    \sans{Flan} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}Dolma 1.7}
        \\[-.4em]
        {\scriptsize\color{darkergrey}decontaminated}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    - &
    8.8 &
    6.7
\\
    \multirow{-2}{*}{\rot{\textbf{\hspace{2em}\scriptsize{INST}}}} &
    \sans{Stack Exchange} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}2024/09/30 dump}
        \\[-.4em]
        {\scriptsize\color{darkergrey}Q\&A format}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    - &
    0.7 &
    0.5
\\
    \rowcolor{ai2offwhite}
    &
    \sans{Starcoder} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    2.1 &
    19.5 &
    20.9 &
    19.2 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite} 
    \multirow{-2}{*}{\rot{\hspace{2em}\textbf{\scriptsize{CODE}}}} &
    \sans{CodeSearchNet} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}unfiltered}\\
    \end{tabular} & 
    - &
    - &
    - &
    - &
    0.1 &
    0.2 &
    0.1
\\
    &
    \sans{Gutenberg Books} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}Dolma 1.7}
    \end{tabular} & 
    - &
    1.2 &
    1.3 &
    1.2 &
    - &
    - &
    -
\\
    &
    \sans{peS2o} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    1.5 &
    6.6 &
    7.1 &
    6.5 &
    10.7 &
    13.0 &
    9.9
\\
    &
    \sans{Wikipedia} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.1 &
    0.9 &
    0.9 &
    0.9 &
    1.6 &
    1.9 &
    1.4
\\
    &
    \sans{StackExchange} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}RedPajama v1}
    \end{tabular} & 
    - &
    4.0 &
    4.3 &
    4.0 &
    - &
    - &
    -
\\
    \multirow{-5}{*}{\rot{\textbf{\hspace{4em}\scriptsize{REFERENCE}}}} &
    \sans{ArXiv} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.5 &
    4.9 &
    5.2 &
    4.8 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}&
    \sans{Algebraic Stack} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.3 &
    2.8 &
    3.0 &
    2.7 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}&
    \sans{OpenWebMath} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.3 &
    2.9 &
    3.1 &
    2.8 &
    5.2 &
    - &
    4.8
\\
    \rowcolor{ai2offwhite}&
    \sans{GSM8k} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}train}
        \\[-.4em]
        {\scriptsize\color{darkergrey}split}
    \end{tabular} & 
    - &
    - &
    0.003 &
    0.003 &
    0.003 &
    - &
    0.003
\\
    \rowcolor{ai2offwhite}&
    \sans{Mathpile} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}commercial subset}
        \\[-.4em]
        {\scriptsize\color{darkergrey}train split}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    2.1 &
    - &
    1.9
\\
    \rowcolor{ai2offwhite}
    \multirow{-5}{*}{\rot{\textbf{\hspace{2.3em}\scriptsize{MATH}}}} &
    \sans{AutoMathText} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}unfiltered}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    18.5 &
    - &
    17.2
\\[.2em]
\bottomrule
\end{tabular}
\end{footnotesize}
\end{center}
\caption{
    A summary of high-quality sources we evaluate for mid-training. 
    We experiment with mixing these sources in 6 mixes, each consisting of 50 billion tokens. 
    Percentages on the table indicate the fraction of each 50B mix that is comprised by data from the respective source. 
    \MeBaseline is sampled (with repetition) from the pretraining stage. 
}
\label{table:hq_mixes}
\end{table}





==> tables/midtrain_results.tex <==
\begin{table}[h]
\centering
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcccc}
\toprule
\textbf{Mid-training mix} & \textbf{OLMES} \sans{(MCF)} & \textbf{OLMES-Gen} & \textbf{MMLU} \sans{(MCF)} & \textbf{GSM*} \\
\midrule
\rowcolor{ai2offwhite}\textit{n/a (pretrain checkpoint)} & 69.6 & 63.2 & 59.8 & 28.5 \\
\MeBaseline & 74.0 & 64.5 & 61.8 & 27.0 \\
\rowcolor{ai2offwhite}\MeDclmSeven & 73.5 & 64.1 & 61.9 & 24.5 \\
\MeFinewebThree & 73.5 & 63.0 & 62.4 & 30.5 \\
\rowcolor{ai2offwhite}\MeFinewebTwo & 75.2 & 63.8 & 63.1 & 28.5 \\
\MeFinewebTwoIns & 74.2 & 64.1 & 63.0 & 46.0 \\
\rowcolor{ai2offwhite}\MeFinewebTwoMath & {\bf75.7} & 69.7 & 62.3 & {\bf52.0} \\
\MeFinewebTwoMathIns & {\bf75.7} & {\bf70.2} & {\bf63.1} & 46.5 \\[.2em]
\bottomrule
\end{tabular}
\end{small}
\caption{
Comparison of mid-training mixes introduced in Table~\ref{table:hq_mixes}. 
Each row corresponds to a 50 billion token training run following learning rate schedule described in Section~\S\ref{sec:learning_rate_deep_dive} (except first row).
Weights are initialized from a \olmotoo checkpoint pretrained for 4T tokens. 
We compare each run on a mix of OLMES core tasks (multiple choice format; see Table~\ref{tab:evals_olmes_mcf}), OLMES generative tasks (Table~\ref{tab:evals_gen}), MMLU (multiple choice format; \citealp{hendryckstest2021}), and a random sample of 200 GSM8K~\citep{cobbe2021trainingverifierssolvemath} questions we use as development set (GSM*; Section~\S\ref{sec:eval-base}).
Results on the {\bf{final mid-training mix}}  are in Table~\ref{tab:evals-pre-post-anneal}.
}
\label{table:hq_mixes_results}
\end{table}

